Bounds on the number of rational points of curves in families

In this note, we give an alternative proof of uniform boundedness of the number of integral points of smooth projective curves over a fixed number field with good reduction outside of a fixed set of primes. We use that due to Bertin-Romagny, the Kodaira-Parshin families constructed by Lawrence-Venkatesh can themselves be assembled into a family. We then repeat Lawrence-Venkatesh's study of the p-adic period map, together with the comparison of nearby fibres.

==> functions.tex <==
\NeedsTeXFormat{LaTeX2e}
%\ProvidesPackage{functions}[Functions via a common preamble]

\newcommand{\z}{\mathbb{Z}} 
\newcommand{\n}{\mathbb{N}}
\newcommand{\co}{\mathbb{C}}
\newcommand{\q}{\mathbb{Q}}
\newcommand{\re}{\mathbb{R}}
\newcommand{\cha}{\text{char}}
\newcommand{\F}{\mathbb{F}}
\newcommand{\A}{\mathbb{A}}
\newcommand{\CRng}{\text{CRng}}
\newcommand{\one}{\mathbbm{1}}
%\newcommand{\rk}{\operatorname{ rk}\hspace{1pt} }
\DeclareMathOperator{\rk}{rk}
\newcommand{\id}{\operatorname{ id}}
\newcommand{\tr}{\operatorname{ tr}}
%\newcommand{\ker}{\operatorname{ ker}}
\newcommand{\im}{\operatorname{ im}}
\newcommand{\cl}{\operatorname{ Cl}}
\newcommand{\Cl}{\operatorname{ Cl}}
\newcommand{\obj}{\operatorname{ Obj}}
\newcommand{\proj}{\operatorname{ Proj}}
\newcommand{\Der}{\operatorname{ Der}}
\newcommand{\Set}{\operatorname{ Set}}
\newcommand{\res}{\operatorname{res}}
\newcommand{\Ind}{\operatorname{Ind}}
\newcommand{\Res}{\text{Res}}
\newcommand{\g}{\mathfrak{g}}
\newcommand{\kf}{\mathfrak{k}}
\newcommand{\Grp}{\text{Grp}}
\newcommand{\p}{\mathfrak{p}}
%\newcommand{\C}{\mathscr{C}}
\newcommand{\ok}{\mathcal{O}_K}
\newcommand{\of}{\mathcal{O}_F}
\newcommand{\ol}{\mathcal{O}_L}
\newcommand{\OO}{\mathcal{O}}
\newcommand{\Nm}{\operatorname{ Nm}}
\newcommand{\SL}{\operatorname{ SL}}
\renewcommand{\sl}{ \mathfrak{sl}}
\newcommand{\GL}{\operatorname{ GL}}
\newcommand{\gl}{ \mathfrak{gl}}
\newcommand{\SO}{\operatorname{ SO}}
\newcommand{\SU}{\operatorname{ SU}}
\newcommand{\Gr}{\operatorname{ Gr}}
\newcommand{\Br}{\operatorname{ Br}}
\newcommand{\gal}{\operatorname{ Gal}}
\newcommand{\Gal}{\operatorname{ Gal}}
\newcommand{\Aut}{\operatorname{ Aut}}
\newcommand{\Div}{\operatorname{ Div}}
\newcommand{\Pic}{\operatorname{ Pic}}
\newcommand{\Spec}{\operatorname{{ Spec}}}
\newcommand{\Spf}{\operatorname{Spf}}
\newcommand{\Hom}{\operatorname{ Hom}}
\newcommand{\uHom}{\underline{\operatorname{ Hom}}}
\newcommand{\Ext}{\operatorname{ Ext}}
\newcommand{\Sel}{\operatorname{ Sel}}
\newcommand{\ind}{\operatorname{ ind}}
\newcommand{\ress}{\operatorname{ res}}
\newcommand{\cores}{\operatorname{ cores}}
\newcommand{\rat}{\operatorname{rat}}
\newcommand{\tors}{\text{tors}}
\newcommand{\coker}{\operatorname{coker}}
\newcommand{\inv}{\operatorname{ inv}}
\newcommand{\fix}{\operatorname{ Fix}}
\newcommand{\hc}{H_{\! \! \text{ \rm cont}}^*}
\newcommand{\htop}{H_{\! \!\text{ \rm top}}^*}
\newcommand{\hgr}{H_{\! \text{ \rm grp}}^*}
\newcommand{\plgr}{P^{\! \text{ \rm grp}}_*}
\newcommand{\hlgr}{H^{\!\text{ \rm grp}}_*}
\newcommand{\hs}{H^*}
\newcommand{\Sch}{\operatorname{ Sch}}
\newcommand{\hls}{H_*}
\newcommand{\hcn}{H_{\! \! \text{ \rm cont}}}
\newcommand{\htopn}{H_{\! \!\text{ \rm top}}}
\newcommand{\hltopn}{H^{\!\text{ \rm top}}}
\newcommand{\hgrn}{H_{\! \!\text{ \rm grp}}}
\newcommand{\plgrn}{P^{\!\text{ \rm grp}}}
\newcommand{\hlgrn}{H^{\!\text{ \rm grp}}}
\newcommand{\lie}{\operatorname{ Lie}}
\newcommand{\st}{\;|\:}
\newcommand{\tss}{\textsuperscript}
\newcommand{\eps}{\epsilon}
\newcommand{\ti}{\times}
\newcommand{\Tr}{\operatorname{ Tr}}
\newcommand{\End}{\operatorname{ End}}
\renewcommand{\L}{\mathcal{L}}
\newcommand{\G}{\mathbb{G}}
\newcommand{\T}{\mathbb{T}}
\newcommand{\FF}{\mathcal{F}}
\newcommand{\Proj}{\text{Proj}}
\newcommand{\Map}{\text{Map}}
\newcommand{\Irr}{\text{Irr}}
\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}
\newcommand{\qq}{\mathfrak{q}}
\newcommand{\s}{\mathfrak{s}}
\newcommand{\D}{\mathscr{D}}
\renewcommand{\AA}{\mathscr{A}}
\newcommand{\Frob}{\text{Frob}}
\newcommand{\Stab}{\text{Stab}}
\newcommand{\opp}{\text{op}}
\newcommand{\h}{\text{h}}
\newcommand{\sh}{\text{sh}}
\newcommand{\etale}{\'{e}tale }
%\newcommand{\et}{\'{e}t}
\newcommand{\unr}{{\rm unr}}
\newcommand{\tame}{{\rm tame}}
\newcommand{\ze}{\zeta}
\renewcommand{\a}{\mathfrak{a}}
\usepackage{letltxmacro}
\LetLtxMacro{\temp}{\phi}
\LetLtxMacro{\phi}{\varphi}
\LetLtxMacro{\varphi}{\temp}


% Text + Styles
\renewcommand{\th}{{\tss{th}} }
\renewcommand{\st}{{\ | \ }}
\newcommand{\ba}{\backslash}

% General Functions

%\DeclareMathOperator*{\sup}{sup}
%\DeclareMathOperator*{\inf}{inf}
\newcommand{\bac}{\backslash}
\newcommand{\pp}{\mathcal{P}}
\newcommand{\R}{\mathcal{R}}

%\newcommand{\End}{\operatorname{End}}
\newcommand{\ab}{\text{ab}}
%\newcommand{\ti}{\times}
\newcommand{\tii}{^\times}
\newcommand{\ot}{\otimes}
\newcommand{\op}{\oplus}
\newcommand{\ord}{\operatorname{ord}}

% Algebra

\newcommand{\PSL}{\operatorname{PSL}}
\newcommand{\Lie}{\operatorname{Lie}}

% Algebraic Number Theory
\newcommand{\Reg}{\operatorname{Reg}}
\newcommand{\cyc}{\text{{\rm cyc}}}
\newcommand{\f}{\mathfrak{f}}
%\newcommand{\ab}{\text{ab}}
%\newcommand{\A}{\mathbb{A}}

% Commutative Algebra

\newcommand{\cor}{\operatorname{cor}}
\newcommand{\zp}{\z_{(p)}}

% Algebraic Geometry
\newcommand{\PP}{\mathbb{P}}
\newcommand{\dR}{\text{dR}}
\newcommand{\HT}{\text{HT}}
\newcommand{\cris}{\text{cris}}
\newcommand{\sta}{\text{st}}
\newcommand{\et}{\text{\'{e}t}}
\renewcommand{\div}{\operatorname{div}}
\newcommand{\Ell}{\text{Ell}}
\newcommand{\GrVHS}{{\mathrm {GrVHS}}}
\newcommand{\GrEt}{{\mathrm{Gr}\acute{\mathrm{E}} \mathrm{t}}}
\newcommand{\MHM}{\mathrm{MHM}}

%\newcommand{\FF}{\mathscr{F}}
\newcommand{\fppf}{\text{fppf}}
\newcommand{\fpqc}{\text{fpqc}}

% Representation Theory

\newcommand{\Lift}{\operatorname{Lift}}
\newcommand{\rti}{\rtimes}
\newcommand{\triv}{\text{{\rm triv}}}
\newcommand{\nt}{\text{{\rm nt}}}
\newcommand{\up}{\!\uparrow}
\newcommand{\down}{\!\downarrow}
\newcommand{\ad}{\text{{\rm ad}}}


% Modular Forms

\newcommand{\hh}{\mathcal{H}}
\newcommand{\M}{\mathcal{M}}
\renewcommand{\SS}{\mathcal{S}}
\newcommand{\Cusps}{\text{Cusps}}
\renewcommand{\S}{\mathbb{S}}

% LaTeX

\def\hyph{-\penalty0\hskip0pt\relax}
\newcommand{\tc}{\textcolor{gray}}
\newcommand{\tcr}{\textcolor{red}}
\newcommand{\tcp}{\textcolor{purple}}
\newcommand{\tco}{\textcolor{orange}}

\endinput
